Study of the long-term Very High Energy emission of the blazars 1ES 1215+3031 and VER J0521+211 with the HAWC gamma-ray observatory

Blazars are the most abundant type of extragalactic gamma-ray source, usually presenting high variability across the electromagnetic spectrum. Their Very High Energy (VHE, above 0.1 TeV) emission has been studied in detail using Air Cherenkov Telescopes, with observations biased to flaring periods while their average activity has not been properly characterized. In this work, we report the results of 2090 days of quasi-continuous observations of the blazars 1ES 1215+303 and VER J0521+211, carried out with the High Altitude Water Cherenkov (HAWC) gamma-ray observatory. Fitting a power-law attenuated by photon-photon interaction with the extragalactic background light, we obtained a 6.2 $\sigma$ level detection for 1ES 1215+303 and a 4.3 $\sigma$ marginal detection for VER J0521+211. With the inclusion of the HAWC TeV spectrum, we built quasi-simultaneous multiwavelength spectral distributions and fitted a leptonic emission model to the observed data.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

